Open Heavy Flavor Studies for the ECCE Detector at the Electron Ion Collider

The ECCE detector has been recommended as the selected reference detector for the future Electron-Ion Collider (EIC). A series of simulation studies have been carried out to validate the physics feasibility of the ECCE detector. In this paper, detailed studies of heavy flavor hadron and jet reconstruction and physics projections with the ECCE detector performance and different magnet options will be presented. The ECCE detector has enabled precise EIC heavy flavor hadron and jet measurements with a broad kinematic coverage. These proposed heavy flavor measurements will help systematically study the hadronization process in vacuum and nuclear medium especially in the underexplored kinematic region.

==> authors/authors-alphabetical.tex <==
%
% Full list of ECCE Collaboratotions
%
% Click Refresh to get the latest version
%
% Goto the following to edit:
% https://www.overleaf.com/1234763137gmqgnzsrpsdj
%

\author[MoreheadState]{J.~K.~Adkins}
\author[RIKEN,RBRC]{Y.~Akiba}
\author[UKansas]{A.~Albataineh}
\author[ODU]{M.~Amaryan}
\author[Oslo]{I.~C.~Arsene}
\author[MSU]{C. Ayerbe Gayoso}
\author[Sungkyunkwan]{J.~Bae}
\author[UVA]{X.~Bai}
\author[BNL,JLab]{M.D.~Baker}
\author[York]{M.~Bashkanov}
\author[UH]{R.~Bellwied}
\author[Duquesne]{F.~Benmokhtar}
\author[CUA]{V.~Berdnikov}
\author[CFNS,StonyBrook,RBRC]{J.~C.~Bernauer}
\author[ORNL]{F.~Bock}
\author[FIU]{W.~Boeglin}
\author[WI]{M.~Borysova}
\author[CNU]{E.~Brash}
\author[JLab]{P.~Brindza}
\author[GWU]{W.~J.~Briscoe}
\author[LANL]{M.~Brooks}
\author[ODU]{S.~Bueltmann}
\author[JazanUniversity]{M.~H.~S.~Bukhari}
\author[UKansas]{A.~Bylinkin}
\author[UConn]{R.~Capobianco}
\author[AcademiaSinica]{W.-C.~Chang}
\author[Sejong]{Y.~Cheon}
\author[CCNU]{K.~Chen}
\author[NTU]{K.-F.~Chen}
\author[NCU]{K.-Y.~Cheng}
\author[BNL]{M.~Chiu}
\author[UTsukuba]{T.~Chujo}
\author[BGU]{Z.~Citron}
\author[CFNS,StonyBrook]{E.~Cline}
\author[NRCN]{E.~Cohen}
\author[ORNL]{T.~Cormier}
\author[LANL]{Y.~Corrales~Morales}
\author[UVA]{C.~Cotton}
\author[CUA]{J.~Crafts}
\author[UKY]{C.~Crawford}
\author[ORNL]{S.~Creekmore}
\author[JLab]{C.Cuevas}
\author[ORNL]{J.~Cunningham}
\author[BNL]{G.~David}
\author[LANL]{C.~T.~Dean}
\author[ORNL]{M.~Demarteau}
\author[UConn]{S.~Diehl}
\author[Yamagata]{N.~Doshita}
\author[IJCLabOrsay]{R.~Dupr\'{e}}
\author[LANL]{J.~M.~Durham}
\author[GSI]{R.~Dzhygadlo}
\author[ORNL]{R.~Ehlers}
\author[MSU]{L.~El~Fassi}
\author[UVA]{A.~Emmert}
\author[JLab]{R.~Ent}
\author[MIT]{C.~Fanelli}
\author[UKY]{R.~Fatemi}
\author[York]{S.~Fegan}
\author[Charles]{M.~Finger}
\author[Charles]{M.~Finger~Jr.}
\author[Ohio]{J.~Frantz}
\author[HUJI]{M.~Friedman}
\author[MIT,JLab]{I.~Friscic}
\author[UH]{D.~Gangadharan}
\author[Glasgow]{S.~Gardner}
\author[Glasgow]{K.~Gates}
\author[Rice]{F.~Geurts}
\author[Rutgers]{R.~Gilman}
\author[Glasgow]{D.~Glazier}
\author[ORNL]{E.~Glimos}
\author[RIKEN,RBRC]{Y.~Goto}
\author[AUGIE]{N.~Grau}
\author[Vanderbilt]{S.~V.~Greene}
\author[IMP]{A.~Q.~Guo}
\author[FIU]{L.~Guo}
\author[Yarmouk]{S.~K.~Ha}
\author[BNL]{J.~Haggerty}
\author[UConn]{T.~Hayward}
\author[GeorgiaState]{X.~He}
\author[MIT]{O.~Hen}
\author[JLab]{D.~W.~Higinbotham}
\author[IJCLabOrsay]{M.~Hoballah}
\author[CUA]{T.~Horn}
\author[AANL]{A.~Hoghmrtsyan}
\author[NTHU]{P.-h.~J.~Hsu}
\author[BNL]{J.~Huang}
\author[Regina]{G.~Huber}
\author[UH]{A.~Hutson}
\author[Yonsei]{K.~Y.~Hwang}
\author[ODU]{C.~E.~Hyde}
\author[Tsukuba]{M.~Inaba}
\author[Yamagata]{T.~Iwata}
\author[Kyungpook]{H.S.~Jo}
\author[UConn]{K.~Joo}
\author[VirginiaUnion]{N.~Kalantarians}
\author[CUA]{G.~Kalicy}
\author[Shinshu]{K.~Kawade}
\author[Regina]{S.~J.~D.~Kay}
\author[UConn]{A.~Kim}
\author[Sungkyunkwan]{B.~Kim}
\author[Pusan]{C.~Kim}
\author[RIKEN]{M.~Kim}
\author[Pusan]{Y.~Kim}
\author[Sejong]{Y.~Kim}
\author[BNL]{E.~Kistenev}
\author[UConn]{V.~Klimenko}
\author[Seoul]{S.~H.~Ko}
\author[MIT]{I.~Korover}
\author[UKY]{W.~Korsch}
\author[UKansas]{G.~Krintiras}
\author[ODU]{S.~Kuhn}
\author[NCU]{C.-M.~Kuo}
\author[MIT]{T.~Kutz}
\author[IowaState]{J.~Lajoie}
\author[JLab]{D.~Lawrence}
\author[IowaState]{S.~Lebedev}
\author[Sungkyunkwan]{H.~Lee}
\author[USeoul]{J.~S.~H.~Lee}
\author[Kyungpook]{S.~W.~Lee}
\author[MIT]{Y.-J.~Lee}
\author[Rice]{W.~Li}
\author[CFNS,StonyBrook,WandM]{W.B.~Li}
\author[USTC]{X.~Li}
\author[CIAE]{X.~Li}
\author[LANL]{X.~Li}
\author[MIT]{X.~Li}
\author[IMP]{Y.~T.~Liang}
\author[Pusan]{S.~Lim}
\author[AcademiaSinica]{C.-h.~Lin}
\author[IMP]{D.~X.~Lin}
\author[LANL]{K.~Liu}
\author[LANL]{M.~X.~Liu}
\author[Glasgow]{K.~Livingston}
\author[UVA]{N.~Liyanage}
\author[WayneState]{W.J.~Llope}
\author[ORNL]{C.~Loizides}
\author[NewHampshire]{E.~Long}
\author[NTU]{R.-S.~Lu}
\author[CIAE]{Z.~Lu}
\author[York]{W.~Lynch}
\author[UNGeorgia]{S.~Mantry}
\author[IJCLabOrsay]{D.~Marchand}
\author[CzechTechUniv]{M.~Marcisovsky}
\author[UoT]{C.~Markert}
\author[FIU]{P.~Markowitz}
\author[AANL]{H.~Marukyan}
\author[LANL]{P.~McGaughey}
\author[Ljubljana]{M.~Mihovilovic}
\author[MIT]{R.~G.~Milner}
\author[WI]{A.~Milov}
\author[Yamagata]{Y.~Miyachi}
\author[AANL]{A.~Mkrtchyan}
\author[CNU]{P.~Monaghan}
\author[Glasgow]{R.~Montgomery}
\author[BNL]{D.~Morrison}
\author[AANL]{A.~Movsisyan}
\author[AANL]{H.~Mkrtchyan}
\author[AANL]{A.~Mkrtchyan}
\author[IJCLabOrsay]{C.~Munoz~Camacho}
\author[UKansas]{M.~Murray}
\author[LANL]{K.~Nagai}
\author[CUBoulder]{J.~Nagle}
\author[RIKEN]{I.~Nakagawa}
\author[UTK]{C.~Nattrass}
\author[JLab]{D.~Nguyen}
\author[IJCLabOrsay]{S.~Niccolai}
\author[BNL]{R.~Nouicer}
\author[RIKEN]{G.~Nukazuka}
\author[UVA]{M.~Nycz}
\author[NRNUMEPhI]{V.~A.~Okorokov}
\author[Regina]{S.~Ore\v{s}i\'{c}}
\author[ORNL]{J.D.~Osborn}
\author[LANL]{C.~O'Shaughnessy}
\author[NTU]{S.~Paganis}
\author[Regina]{Z.~Papandreou}
\author[NMSU]{S.~F.~Pate}
\author[IowaState]{M.~Patel}
\author[MIT]{C.~Paus}
\author[Glasgow]{G.~Penman}
\author[UIUC]{M.~G.~Perdekamp}
\author[CUBoulder]{D.~V.~Perepelitsa}
\author[LANL]{H.~Periera~da~Costa}
\author[GSI]{K.~Peters}
\author[CNU]{W.~Phelps}
\author[TAU]{E.~Piasetzky}
\author[BNL]{C.~Pinkenburg}
\author[Charles]{I.~Prochazka}
\author[LehighUniversity]{T.~Protzman}
\author[BNL]{M.~L.~Purschke}
\author[WayneState]{J.~Putschke}
\author[MIT]{J.~R.~Pybus}
\author[JLab]{R.~Rajput-Ghoshal}
\author[ORNL]{J.~Rasson}
\author[FIU]{B.~Raue}
\author[ORNL]{K.F.~Read}
\author[Oslo]{K.~R\o{}ed}
\author[LehighUniversity]{R.~Reed}
\author[FIU]{J.~Reinhold}
\author[LANL]{E.~L.~Renner}
\author[UConn]{J.~Richards}
\author[UIUC]{C.~Riedl}
\author[BNL]{T.~Rinn}
\author[Ohio]{J.~Roche}
\author[MIT]{G.~M.~Roland}
\author[HUJI]{G.~Ron}
\author[IowaState]{M.~Rosati}
\author[UKansas]{C.~Royon}
\author[Pusan]{J.~Ryu}
\author[Rutgers]{S.~Salur}
\author[MIT]{N.~Santiesteban}
\author[UConn]{R.~Santos}
\author[GeorgiaState]{M.~Sarsour}
\author[ORNL]{J.~Schambach}
\author[GWU]{A.~Schmidt}
\author[ORNL]{N.~Schmidt}
\author[GSI]{C.~Schwarz}
\author[GSI]{J.~Schwiening}
\author[RIKEN,RBRC]{R.~Seidl}
\author[UIUC]{A.~Sickles}
\author[UConn]{P.~Simmerling}
\author[Ljubljana]{S.~Sirca}
\author[GeorgiaState]{D.~Sharma}
\author[LANL]{Z.~Shi}
\author[Nihon]{T.-A.~Shibata}
\author[NCU]{C.-W.~Shih}
\author[RIKEN]{S.~Shimizu}
\author[UConn]{U.~Shrestha}
\author[NewHampshire]{K.~Slifer}
\author[LANL]{K.~Smith}
\author[Glasgow,CEA]{D.~Sokhan}
\author[LLNL]{R.~Soltz}
\author[LANL]{W.~Sondheim}
\author[CIAE]{J.~Song}
\author[Pusan]{J.~Song}
\author[GWU]{I.~I.~Strakovsky}
\author[BNL]{P.~Steinberg}
\author[CUA]{P.~Stepanov}
\author[WandM]{J.~Stevens}
\author[PNNL]{J.~Strube}
\author[CIAE]{P.~Sun}
\author[CCNU]{X.~Sun}
\author[Regina]{K.~Suresh}
\author[AANL]{V.~Tadevosyan}
\author[NCU]{W.-C.~Tang}
\author[IowaState]{S.~Tapia~Araya}
\author[Vanderbilt]{S.~Tarafdar}
\author[BrunelUniversity]{L.~Teodorescu}
\author[UoT]{D.~Thomas}
\author[UH]{A.~Timmins}
\author[CzechTechUniv]{L.~Tomasek}
\author[UConn]{N.~Trotta}
\author[CUA]{R.~Trotta}
\author[Oslo]{T.~S.~Tveter}
\author[IowaState]{E.~Umaka}
\author[Regina]{A.~Usman}
\author[LANL]{H.~W.~van~Hecke}
\author[IJCLabOrsay]{C.~Van~Hulse}
\author[Vanderbilt]{J.~Velkovska}
\author[IJCLabOrsay]{E.~Voutier}
\author[IJCLabOrsay]{P.K.~Wang}
\author[UKansas]{Q.~Wang}
\author[CCNU]{Y.~Wang}
\author[Tsinghua]{Y.~Wang}
\author[York]{D.~P.~Watts}
\author[CUA]{N.~Wickramaarachchi}
\author[ODU]{L.~Weinstein}
\author[MIT]{M.~Williams}
\author[LANL]{C.-P.~Wong}
\author[PNNL]{L.~Wood}
\author[CanisiusCollege]{M.~H.~Wood}
\author[BNL]{C.~Woody}
\author[MIT]{B.~Wyslouch}
\author[Tsinghua]{Z.~Xiao}
\author[KobeUniversity]{Y.~Yamazaki}
\author[NCKU]{Y.~Yang}
\author[Tsinghua]{Z.~Ye}
\author[Yonsei]{H.~D.~Yoo}
\author[LANL]{M.~Yurov}
\author[York]{N.~Zachariou}
\author[Columbia]{W.A.~Zajc}
\author[USTC]{W.~Zha}
\author[SDU]{J.-L.~Zhang}
\author[UVA]{J.-X.~Zhang}
\author[Tsinghua]{Y.~Zhang}
\author[IMP]{Y.-X.~Zhao}
\author[UVA]{X.~Zheng}
\author[Tsinghua]{P.~Zhuang}


==> header.tex <==


\RequirePackage{lineno}
\input{institute_list}
\usepackage{import}
%\usepackage{titlesec}
\usepackage{enumitem}
\usepackage{amssymb, amsmath}
\usepackage{mathpazo}
\usepackage{float,graphicx}
%\graphicspath{{./}{pCDR/}}
\usepackage[figuresright]{rotating}
\usepackage{wrapfig}
\usepackage[usenames,dvipsnames]{color}
\usepackage{microtype}
\usepackage{tabulary}
%\usepackage{booktabs,multirow,dcolumn,bigdelim}
\newcommand{\otoprule}{\midrule[\heavyrulewidth]}
\usepackage{xr-hyper}
\usepackage[pdftex,plainpages=false,pdfpagelabels,backref,pdfborder={0 0 0}]{hyperref}
%\usepackage{hyperref}
\usepackage{authblk}
\usepackage{url}
\usepackage[toc,page,titletoc]{appendix}
%\usepackage{afterpage}
\usepackage[font=small,labelfont=bf]{caption}
\setlength\captionmargin{15pt}
\usepackage[scaled]{helvet}
\usepackage{sectsty}
\allsectionsfont{\normalfont\sffamily}
%\usepackage{titletoc}
\usepackage{bytefield}
\usepackage{verbatimbox}
\usepackage{tabularx}

%\titlecontents{chapter}
%  [1.5em]
%  {\linespread{0.9}\normalfont\sffamily\bfseries}
%  {\contentslabel{1em}} 
%  {\hspace*{-1.3em}} 
%  {\mdseries\titlerule*[1pc]{.}\contentspage} 
%\titlecontents{section}
%  [3.5em]
%  {\linespread{0.9}\normalfont\sffamily}
%  {\contentslabel{2.3em}} 
%  {\hspace*{-2.3em}} 
%  {\titlerule*[1pc]{.}\contentspage} 
%\titlecontents{subsection}
%  [4.5em]
%  {\linespread{0.9}\normalfont\sffamily}
%  {\contentslabel{2.3em}} 
%  {\hspace*{-2.3em}} 
%  {\titlerule*[1pc]{.}\contentspage} 
%\titlecontents{subsubsection}
%  [5.5em]
%  {\linespread{0.9}\normalfont\sffamily}
%  {\contentslabel{2.3em}} 
%  {\hspace*{-2.3em}} 
%  {\titlerule*[1pc]{.}\contentspage} 
%\tolerance = 10000

\usepackage[text={6.5in,8.75in},headheight=26pt,centering]{geometry}
\usepackage{xspace}

\DeclareGraphicsExtensions{.pdf,.png}
\newcommand{\filenamedot}{.}
\setlength{\parindent}{0.0in}
\setlength{\parskip}{0.1in}
\renewcommand{\topfraction} {0.9}
\renewcommand{\bottomfraction} {0.9}
\renewcommand{\textfraction} {0.1}
\renewcommand{\floatpagefraction} {0.8}

%\usepackage{fancyhdr}
%\pagestyle{fancy}
%\renewcommand{\chaptermark}[1]{\markboth{#1}{}}
%\renewcommand{\sectionmark}[1]{\markright{#1}{}}
%\fancyhead{} % clear all header fields 
%\fancyhead[RO,LE]{\sffamily \rightmark}
%\fancyhead[LO,RE]{\sffamily \leftmark}
%\fancyfoot{} % clear all footer fields 
%\fancyfoot[RO,LE]{\sffamily \thepage}
%\renewcommand{\headrulewidth}{0pt} 
%\fancypagestyle{plain}{%
%  \fancyhf{}
%  \fancyfoot[RO,LE]{\sffamily \thepage}
%}

\usepackage{multirow}
\usepackage{eurosym}
\usepackage{xcolor}
\usepackage{framed}
\colorlet{shadecolor}{blue!10}

\usepackage{gensymb}

\setcounter{secnumdepth}{3}

\def\consortium{ECCE consortium}
\newcommand{\martinimusic}{\mbox{\sc Martini+Music}\xspace}
\newcommand{\hic}{\mbox{$A$$+$$A$}\xspace}
\newcommand{\pA}{\mbox{$p$$+$$A$}\xspace}
\newcommand{\AuAu}{\mbox{Au$+$Au}\xspace}
\newcommand{\auau}{\mbox{Au$+$Au}\xspace} 
\newcommand{\raa}{\mbox{$R_\mathrm{AA}$}\xspace}
\newcommand{\pbpb}{\mbox{Pb$+$Pb}\xspace} 
\newcommand{\pdau}{\mbox{$p(d)$$+$Au}\xspace} 
\newcommand{\pau}{\mbox{$p$$+$Au}\xspace} 
\newcommand{\aj}{\mbox{$A_J$}\xspace} 
\newcommand {\pp}{\mbox{$p$$+$$p$}\xspace}
\newcommand {\ppbar}{\mbox{$p$$+$$\overline{p}$}\xspace}
\newcommand{\pT}{\mbox{${p_T}$}\xspace}
\newcommand{\jpsi}{\mbox{$J/\psi$}}
\newcommand{\sqrtsnn}{\mbox{$\sqrt{s_{\scriptscriptstyle NN}}$}}
\newcommand{\npart}{$N_\mathrm{part}$}
\newcommand{\ncoll}{$N_\mathrm{coll}$}
\newcommand{\qgp}{\mbox{quark-gluon plasma}\xspace}
\newcommand{\jt}{\mbox{$J_T$}} \newcommand{\qhat}{\mbox{$\hat{q}$}}
\newcommand{\Qsqr}{\mbox{$Q^2$}} \newcommand{\CuCu}{\mbox{Cu$+$Cu}}
\newcommand{\PbPb}{\mbox{Pb$+$Pb}} \newcommand{\pPb}{\mbox{$p$$+$Pb}}
\newcommand{\gjet}{\mbox{$\gamma$-jet}}
\newcommand{\Qmax}{\mbox{$Q_{\max}$}} \newcommand{\ET}{\mbox{$E_T$}}
\newcommand{\Et}{\mbox{$E_T$}} \newcommand{\kt}{\mbox{$k_T$}}
\newcommand{\RAA}{\mbox{$R_{AA}$}\xspace} \newcommand{\IAA}{\mbox{$I_{AA}$}}
\newcommand{\pt}{\mbox{${p_T}$}\xspace}
\newcommand{\highpt}{high-${\rm p_{_{T}}}$}
\newcommand{\lessim}{{\stackrel{<}{\sim}}} \newcommand{\eqnpt}{p_T}
\newcommand{\eA}{\mbox{$e-{\rm A}$}}
\newcommand{\dAu}{\mbox{$d$$+$Au}\xspace}
\newcommand{\pAu}{\mbox{$p$$+$Au}\xspace}
\newcommand{\GeVSQ}{\mbox{${\rm GeV}^2$}}
\newcommand{\fastjet}{\mbox{\sc FastJet}\xspace}
\newcommand{\geant}{\mbox{\sc Geant4}\xspace}
\newcommand{\antikt}{\mbox{anti-$k_T$}\xspace}
\newcommand{\pythia}{\mbox{\sc Pythia}\xspace}
\newcommand{\opera}{\mbox{\sc Opera}\xspace}
\newcommand{\rapgap}{\mbox{\sc Rapgap}\xspace}
\newcommand{\milou}{\mbox{\sc Milou}\xspace}
\newcommand{\pyquen}{\mbox{\sc Pyquen}\xspace}
\newcommand{\hijing}{\mbox{\sc Hijing}\xspace}
\newcommand{\roofit}{\mbox{\sc RooFit}\xspace}
\newcommand{\roounfold}{\mbox{\sc RooUnfold}\xspace}
\newcommand{\beetle}{\mbox{\sc Beetle}\xspace}
\newcommand{\gj}{\mbox{$\gamma$+jet}\xspace}
\newcommand{\gh}{\mbox{$\gamma$+hadron}\xspace}
\newcommand{\martini}{\mbox{\sc Martini}\xspace}
\newcommand{\music}{\mbox{\sc Music}\xspace}

\newcommand{\refdesign}{reference design\xspace}
\newcommand{\refconfig}{reference configuration\xspace}
\newcommand{\dijet}{\mbox{dijet}\xspace}
\newcommand{\fake}{\mbox{fake}\xspace}
\newcommand{\fast}{\mbox{fast}\xspace}
\newcommand{\veryfast}{\mbox{very fast}\xspace}
\newcommand{\epem}{\mbox{$e^+e^-$}\xspace}
\newcommand{\onewidth}{0.6\linewidth}
\newcommand{\twowidth}{0.48\linewidth}
\newcommand{\threewidth}{0.32\linewidth}
\newcommand{\egoing}{\mbox{electron-going}\xspace}
\newcommand{\hgoing}{\mbox{hadron-going}\xspace}
\newcommand{\egodir}{electron-going direction\xspace}
\newcommand{\hgodir}{hadron-going direction\xspace}

\newcommand{\red}{\color{red}}
\newcommand{\blue}{\color{blue}}	 
\newcommand{\green}{\color{green}}	 
\newcommand{\magenta}{\color{magenta}}

\newcommand{\lyxdot}{.}
\usepackage{subfig}

\setlength\fboxsep{0pt}
\setlength\fboxrule{0.5pt}

\usepackage[textwidth=1in,textsize=footnotesize,disable]{todonotes}
%\usepackage[textwidth=1in,textsize=footnotesize]{todonotes}

